Adaptive multigrid for high-order discontinuous Galerkin methods based on the full approximation scheme

We propose an adaptive multigrid (MG) method for discontinuous Galerkin formulations of elliptic problems using Brandt's full approximation scheme (FAS). Unlike common approaches, this method achieves local $hp$-refinement of hexahedral meshes without the need for hanging nodes. The core component of the FAS-MG method is an overlapping Schwarz smoother, which is optionally accelerated by a Krylov method. This smoother is designed for unstructured curvilinear meshes but maintains a tensor-product structure for fast diagonalization. Numerical experiments demonstrate the exceptional efficiency of the FAS-MG method. Dedicated studies confirm its robustness against high aspect ratios, element deformation, and irregular mesh topology. We also verify its capability for dynamic parallel mesh adaptation using the wave-front benchmark of \v{C}erven\'y, Dobrev, and Kolev (SIAM J. Sci. Comp. 41, 2019). Finally, we present preliminary results of extending the method to incompressible Navier-Stokes problems.

==> def.tex <==
% !TEX encoding = UTF-8 Unicode
% !TEX root = dg-mg.tex

%% Math %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% import double braces from stix
\makeatletter
\@ifpackageloaded{stix}{%
}{%
  \DeclareFontEncoding{LS2}{}{\noaccents@}
  \DeclareFontSubstitution{LS2}{stix}{m}{n}
  \DeclareSymbolFont{stix@largesymbols}{LS2}{stixex}{m}{n}
  \SetSymbolFont{stix@largesymbols}{bold}{LS2}{stixex}{b}{n}
  \DeclareMathDelimiter{\lBrace}{\mathopen} {stix@largesymbols}{"E8}%
                                            {stix@largesymbols}{"0E}
  \DeclareMathDelimiter{\rBrace}{\mathclose}{stix@largesymbols}{"E9}%
                                            {stix@largesymbols}{"0F}
}
\makeatother


\newcommand {\mathsc}[1]{\text{{\sffamily\scshape #1}}}

\newcommand {\fc}  {\M f_\mathrm{c}}
\newcommand {\hc}  {\M h_\mathrm{c}}
\newcommand {\fd}  {\M f_\mathrm{d}}
\newcommand {\fs}  [1][] {\M f_\mathrm{s #1}}

\newcommand {\Ad}  {\M A_\mathrm{d}}


\newcommand {\PO}  {\mathcal M}
\newcommand {\Fc}  {\mathcal F_{\!\mathrm{c}}}
\newcommand {\Fd}  {\mathcal F_{\!\mathrm{d}}}
\newcommand {\Fs}  {\mathcal F_{\!\mathrm{s}}}
\newcommand {\Sd}  {\mathcal S_{\!\mathrm{d}}}

\newcommand {\iu}  {\mathrm{i}}
\newcommand {\zi}  {z_\mathrm{i}}
\newcommand {\zr}  {z_\mathrm{r}}

\newcommand {\V}  [1] {\bm{#1}}                        % physical vector
\newcommand {\T}  [1] {\bm{#1}}                        % tensor field
\newcommand {\TS} [1] {\bm{#1}}                        % tensor field (greek)
\newcommand {\TC} [1] {\mathbf{#1}}                    % tensor constant
\newcommand {\M}  [1] {\bm{#1}}                        % matrix
\newcommand {\MC} [1] {\mathbf{#1}}                    % matrix constant

\newcommand {\NM} [1] {\underaccent{\bar}{#1}}         % nodal matrix
\newcommand {\NMC}[1] {\underaccent{\bar}{\mathrm #1}} % nodal matrix constant
%\newcommand {\NMV}[1] {\underaccent{\bar}{\V #1}}      % nodal matrix of vectors



\providecommand {\abs} [1] {\left\vert#1\right\vert}
\providecommand {\norm}[1] {\left\Vert#1\right\Vert}
\providecommand {\seminorm} [1] {\abs{#1}}

\renewcommand {\d}            {\partial}
\newcommand   {\D}            {\mathrm{d}\mspace{1.0mu}}
%\newcommand   {\sgn}          {\operatorname{sgn}}
\newcommand   {\diag}         {\operatorname{diag}}
%\newcommand   {\imag}     [1] {\operatorname{Im}(#1)}
%\newcommand   {\real}     [1] {\operatorname{Re}(#1)}
\newcommand   {\transpose}[1] {#1^{t}}
\newcommand   {\jmp}      [1] {\left\lBrack #1\right\rBrack}   % with stix
\newcommand   {\avg}      [1] {\left\lBrace #1\right\rBrace}   % with stix 

\newcommand{\n} [2][] {n_{\textsc{#2} #1}}
\newcommand{\N} [2][] {N_{\textsc{#2} #1}}


%% Theorems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{remark}{Remark}



==> num-exp-overlap.tex <==
      &         $\delta$
 $p$  &  0.04  &  0.08  &  0.16
  4   &    1   &    1   &    1
  8   &    1   &    2   &    2
 16   &    2   &    3   &    5
 32   &    4   &    6   &    6



